Cross-lingual Transfer Can Worsen Bias in Sentiment Analysis

Sentiment analysis (SA) systems are widely deployed in many of the world's languages, and there is well-documented evidence of demographic bias in these systems. In languages beyond English, scarcer training data is often supplemented with transfer learning using pre-trained models, including multilingual models trained on other languages. In some cases, even supervision data comes from other languages. Does cross-lingual transfer also import new biases? To answer this question, we use counterfactual evaluation to test whether gender or racial biases are imported when using cross-lingual transfer, compared to a monolingual transfer setting. Across five languages, we find that systems using cross-lingual transfer usually become more biased than their monolingual counterparts. We also find racial biases to be much more prevalent than gender biases. To spur further research on this topic, we release the sentiment models we used for this study, and the intermediate checkpoints throughout training, yielding 1,525 distinct models; we also release our evaluation code.

==> figures/all_results.tex <==
% TODO work out how to put the language labels and the bias types on them without lots of captions? OR maybe captions are good.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_ja_gender.pdf}
        \caption{Japanese (ja) - Gender}
        \label{fig:ja_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_ja_race.pdf}
        \caption{Japanese (ja) - Race}
        \label{fig:ja_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_zh_gender.pdf}
        \caption{Chinese (zh) - Gender}
        \label{fig:zh_gender}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_de_gender.pdf}
        \caption{German (de) - Gender}
        \label{fig:de_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_de_race.pdf}
        \caption{German (de) - Race}
        \label{fig:de_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_es_gender.pdf}
        \caption{Spanish (es) - Gender}
        \label{fig:es_gender}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_es_race.pdf}
        \caption{Spanish (es) - Race}
        \label{fig:es_race}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_en_gender.pdf}
        \caption{English (en) - Gender}
        \label{fig:en_gender}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models/all_models_en_race.pdf}
        \caption{English (en) - Race}
        \label{fig:en_race}
    \end{subfigure}
    % TODO can I put en_scrubbed on the same graph as en? Have either 8 or 10 graphs depending which...

    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Mean and variance of difference in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}). Monolingual models are trained and tested on the same language, multilingual models are pretrained multilingual models where the classification layer is trained on English and then zero shot to the target language.} 
    \label{fig:all_results}
\end{figure*}


% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.348\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_baseline.pdf}
%         \caption{Baseline (monolingual) models}
%         \label{fig:baseline_results}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_mono.pdf}
%         \caption{Monolingual models}
%         \label{fig:mono_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_multi.pdf}
%         \caption{Multilingual models}
%         \label{fig:multi_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
   
%     \caption{Mean performance gap between privileged and minoritized groups, by language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias. Languages are ISO codes, with \textit{en\_s} for English (scrubbed). Points that are not statistically significant ($\alpha < 0.05$) are included but marked with an X. Monolingual models are trained and tested on the same language, multilingual model are pretrained mbert models where the classification layer is trained on English and then zero shot to the target language.} 
%     \label{fig:all_results}
% \end{figure*}


==> figures/all_results_violin.tex <==
% TODO work out how to put the language labels and the bias types on them without lots of captions? OR maybe captions are good.
\begin{figure*}[t!]
    \centering
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_ja_gender.pdf}
        \caption{Japanese (ja) - Gender}
        \label{fig:ja_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_ja_race.pdf}
        \caption{Japanese (ja) - Race}
        \label{fig:ja_race_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_zh_gender.pdf}
        \caption{Chinese (zh) - Gender}
        \label{fig:zh_gender_violin}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_de_gender.pdf}
        \caption{German (de) - Gender}
        \label{fig:de_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_de_race.pdf}
        \caption{German (de) - Race}
        \label{fig:de_race_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_es_gender.pdf}
        \caption{Spanish (es) - Gender}
        \label{fig:es_gender_violin}
    \end{subfigure}


    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_en_gender.pdf}
        \caption{English (en) - Gender}
        \label{fig:en_gender_violin}
    \end{subfigure}
    \begin{subfigure}[b]{0.325\textwidth}
        \includegraphics[width=\textwidth]{figures/all_models_violin/all_models_en_race.pdf}
        \caption{English (en) - Race}
        \label{fig:en_race_violin}
    \end{subfigure}
    % TODO can I put en_scrubbed on the same graph as en? Have either 8 or 10 graphs depending which...

    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Violin plots of the distribution of differences in sentiment label under each counterfactual (range is -4 to 4 since labels range from 1 to 5). Higher numbers indicate greater bias against the minoritized group, 0 indicates invariance to the counterfactual. Monolingual models are trained and tested on the same language, multilingual models are pretrained multilingual models where the classification layer is trained on English and then zero shot to the target language.} 
    \label{fig:all_results_violin}
\end{figure*}


% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.348\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_baseline.pdf}
%         \caption{Baseline (monolingual) models}
%         \label{fig:baseline_results}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_mono.pdf}
%         \caption{Monolingual models}
%         \label{fig:mono_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%       %(or a blank line to force the subfigure onto a new line)
%     \begin{subfigure}[b]{0.31\textwidth}
%         \includegraphics[width=\textwidth]{figures/all_data_multi.pdf}
%         \caption{Multilingual models}
%         \label{fig:multi_results}
%     \end{subfigure}
%     ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
%     %(or a blank line to force the subfigure onto a new line)
   
%     \caption{Mean performance gap between privileged and minoritized groups, by language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias. Languages are ISO codes, with \textit{en\_s} for English (scrubbed). Points that are not statistically significant ($\alpha < 0.05$) are included but marked with an X. Monolingual models are trained and tested on the same language, multilingual model are pretrained mbert models where the classification layer is trained on English and then zero shot to the target language.} 
%     \label{fig:all_results}
% \end{figure*}


==> figures/baseline_mono_confusion_matrix.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.48\textwidth]{figures/confusion_matrix/baseline_mono_heatmap.pdf}
    \caption{Confusion matrices for racial demographic counterfactual pairs for Japanese and German, comparing the difference between baseline and monolingual transfer (mono-T) models (RQ1). Higher colour saturation in the lower triangle is bias against the minoritised group, in the upper triangle is bias against the privileged group. Other languages and bias types follow the same pattern between baseline and mono-T models (regardless of absolute level of bias).} 
    \label{fig:baseline_mono_conf_matrix}
    \vspace{-1em}
\end{figure}

==> figures/baseline_mono_confusion_matrix_old.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_race_baseline_cap.pdf}
        \caption{Japanese (ja) Baseline}
        \label{fig:ja_race_baseline_conf}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_race_mono_cap.pdf}
        \caption{Japanese (ja) Mono-T}
        \label{fig:ja_race_mono_conf}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
   
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/de_race_baseline_cap.pdf}
        \caption{German (de) Baseline}
        \label{fig:de_race_baseline_conf}
    \end{subfigure}
    \begin{subfigure}[b]{0.35\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/de_race_mono_cap.pdf}
        \caption{German (de) Mono-T}
        \label{fig:de_race_mono_conf}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
    \caption{Confusion matrices for racial demographic counterfactual pairs for Japanese and German, comparing the difference between baseline and monolingual transfer (Mono-T) models. Higher colour saturation in the lower triangle is bias against the minoritised group, in the upper triangle is bias against the privileged group. Data along the matrix diagonal (invariance under the counterfactual) has been removed to make interpretation clearer, as even in the most biased models many samples are invariant. Other languages and bias types follow the same pattern between baseline and Mono-T models (regardless of absolute level of bias).} 
    \label{fig:baseline_mono_conf_matrix}
    \vspace{-1em}
\end{figure*}


%ig:baseline_mono_conf_matrix

==> figures/baseline_mono_confusion_matrix_short_paper.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.40\textwidth]{figures/confusion_matrix/baseline_mono_heatmap.pdf}
    \caption{Confusion matrices for racial counterfactual pairs for Japanese and German, comparing baseline and pretrained models. Higher colour saturation in the lower triangle is bias against the minoritised group, against the privileged group in the upper triangle. 
    % Other languages and bias types follow the same pattern between baseline and mono-T models (regardless of absolute level of bias).
    } 
    \label{fig:baseline_mono_conf_matrix}
    \vspace{-1em}
\end{figure}

==> figures/baseline_vs_mono.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/baseline_mono_gender.pdf}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\textwidth}
        \includegraphics[width=\textwidth]{figures/baseline_mono_race.pdf}
    \end{subfigure}
   
    \caption{Aggregate bias metrics for baseline (blue), pretrained mono-T (orange), and pretrained distil mono-T (green) models. Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}). Spanish (es) distilled model is intentionally missing for lack of comparable pretrained model.} 
    \label{fig:baseline_vs_mono}
    \vspace{-1em}
\end{figure*}


==> figures/baseline_vs_mono_old.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/baseline_vs_mono_agg.pdf}
    \caption{Aggregate bias metrics for baseline (blue), mono-T (orange), and distil mono-T (green) models: mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:baseline_vs_mono_old}
    \vspace{-1em}
\end{figure*}


==> figures/en_scrubbed_results.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{figures/compare_langs/compare_langs_en_en_scrubbed_gender_errbars.pdf}
        \caption{Mean and variance of the performance gaps for the gender counterfactuals in monolingual models of English (O) and scrubbed English (X). Positive numbers are bias against the minoritised group (in this case, female), 0 is no bias, and negative is bias against the privileged group. Shaded region represents 3\% of total range (see \ref{sec:metrics}).}
        \label{fig:en_scrubbed_errbars}
    \end{subfigure}
    \begin{subfigure}[b]{0.46\textwidth}
        \includegraphics[width=\textwidth]{figures/compare_langs/compare_langs_en_en_scrubbed_baseline_gender.pdf}
        \caption{Difference between confusion matrices of the gender counterfactual for English and scrubbed English baseline model (male demographic labels on x axis, female demographic counterfactual on y). The diagonal represents no bias in either direction, the upper right is bias against men, the lower left is bias against women. Red cells mean the English model has more, blue mean the scrubbed English model has more, and white mean their numbers are identical.}
        \label{fig:diff_matrix_en_scrubbed}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Comparisons of gender bias for English and English with explicit gender identifiers removed (aka "scrubbed" English). Scrubbing increases bias in the baseline, but does not much change either neural model.} 
    \label{fig:en_scrubbed_experiments}
\end{figure}


==> figures/fig_template.tex <==
\begin{figure*}[ht]
    \centering
    \begin{subfigure}[b]{0.348\textwidth}
        \includegraphics[width=\textwidth]{figures/X.pdf}
        \caption{}
        \label{fig:b}
    \end{subfigure}
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/Y.pdf}
        \caption{}
        \label{fig:}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
      %(or a blank line to force the subfigure onto a new line)
    \begin{subfigure}[b]{0.31\textwidth}
        \includegraphics[width=\textwidth]{figures/X.pdf}
        \caption{}
        \label{fig:}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{} 
    \label{fig:}
\end{figure*}


==> figures/front_example_short.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figures/front_example_short_horizontal.pdf}
    \caption{We create corpora and then do counterfactual evaluation to evaluate how bias is transferred from training data. Counterfactual pairs (e.g. sentences \textit{a}, \textit{b}) vary a single demographic variable (e.g. race). We measure bias as the difference in scores for the pair. An unbiased model should be invariant to the counterfactual, with a difference of zero.}
    \label{fig:front_example}
    \vspace{-1em}
\end{figure}

==> figures/label_bal_confusion.tex <==
\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{0.215\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_gender_multi_xl_c_cap.pdf}
        \caption{distil ZS-XLT* (not balanced)}
        \label{fig:distilZSXLT_confusion}
    \end{subfigure}
    \begin{subfigure}[b]{0.215\textwidth}
        \includegraphics[width=\textwidth]{figures/confusion_matrix/ja_gender_multi_xl_c_b_cap.pdf}
        \caption{distil ZS-XLT (balanced)}
        \label{fig:distilZSXLT_balanced_confusion}
    \end{subfigure}
    ~ %add desired spacing between images, e. g. ~, \quad, \qquad, \hfill etc. 
    %(or a blank line to force the subfigure onto a new line)
   
    \caption{Confusion matrices for gender counterfactual pairs for Japanese, comparing the difference between a model trained with imbalanced and balanced labels. Higher colour saturation in the lower triangle is anti-female bias, in the upper is anti-male. Data along the matrix diagonal (no change under counterfactual) has been removed to make interpretation clearer. Other languages and bias types follow the same visual pattern of the matrix between balanced and imbalanced labels, regardless of of distillation and of absolute level of bias.} 
    \label{fig:label_balancing_confusion}
    \vspace{-1em}
\end{figure}


==> figures/mono_vs_multi_old.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/mono_vs_multi_agg.pdf}
    \caption{Aggregate bias metrics for mono-T (blue), and mono-XLT (orange), ZS-XLT (green), distil mono-T (red), and distil ZS-XLT (purple) models. Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:mono_vs_multi_old}
    \vspace{-1em}
\end{figure*}


==> figures/normal_vs_balanced.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{figures/label_bal_agg.pdf}
    \caption{Aggregate bias metrics for label balancing experiments:. Mean and variance of differences in the sentiment label under each counterfactual pair, one graph per language and type of bias tested. Higher numbers indicate greater bias against the minoritized group. The dashed line at zero indicates no bias, the shaded region corresponds to 3\% of total range (see \ref{sec:metrics}).} 
    \label{fig:normal_vs_balanced}
    \vspace{-1em}
\end{figure*}


==> tables/bias_corpora.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{ccc} \toprule
        & Gender & Race/Immigrant  \\
        \midrule
         Japanese & 3340 & 2004 \\
         Chinese & 4928 &  - \\
         German & 3200 & 5236 \\
         Spanish & 4240 & 6360 \\
         English & 2880 & 5760 \\ \bottomrule
    \end{tabular}
    \caption{Counterfactual pairs in each evaluation set, including original reference English. Differences in corpus size are due to differing number of grammatical variants and demographic words across languages.}
    \label{tab:bias_corpora}
    \vspace{-1em}
\end{table}

==> tables/in_domain_performance.tex <==
% !TEX root = ../acl.tex


\begin{table}[h]
\adjustbox{max width=0.5\textwidth}{%
\centering
\begin{tabular}{lllllll}
& \multicolumn{2}{c}{\textbf{Standard}}  & \multicolumn{2}{c}{\textbf{Distilled}}  & \multicolumn{2}{c}{\textbf{Baseline}} \\
& F1 & Steps & F1 & Steps & F1 \\
\toprule
ja & \textbf{0.62} & 44370 & 0.61 & 60436 & 0.38 \\
zh & \textbf{0.56} & 35190 & 0.53 & 43750 & 0.42 \\
de & \textbf{0.63} & 36720 & 0.63 & 52621 & 0.51 \\
es & \textbf{0.61} & 41310 &  & - & 0.48 \\
en & \textbf{0.65} & 27050 & \textbf{0.65} & 44285 & 0.53 \\
%en\_s & \textbf{0.65} & 26520 & 0.64 & 17193 & 0.52 \\
%multi & \textbf{0.71} & 100644 & 0.70 & 78280 & - \\
%ZS-XLT & \textbf{0.69} & 75000 & 0.68 & 33336 & - \\

\bottomrule
\end{tabular}
}
    \caption{F1 at convergence and steps at convergence for standard size, distilled, and baseline models. Performance is measured on the MARC data.}
    \label{tab:in_domain_performance}
\end{table}


==> tables/tab_template.tex <==
% !TEX root = ../acl.tex


\begin{table}[h]
\adjustbox{max width=\textwidth}{%
\centering
\begin{tabular}{lllllll}
& X & Y \\
\toprule
ja &  &  &  & &  & \\
zh &  &  &  & &  & \\
de &  &  &  & &  & \\
es &  &  &  & &  & \\
en &  &  &  & &  & \\
en_s &  &  &  & &  & \\
multi &  &  &  & &  & \\
multi-bal &  &  &  & &  & \\

\bottomrule
\end{tabular}
}
    \caption{Blah}
    \label{tab:}
\end{table}
